Magnetic field sensors using 13-spin cat states

Measurement devices could benefit from entangled correlations to yield a measurement sensitivity approaching the physical Heisenberg limit. Building upon previous magnetometric work using pseudo-entangled spin states in solution-state NMR, we present two conceptual advancements to better prepare and interpret the pseudo-entanglement resource as well as the use of a 13-spin cat state to measure the local magnetic field with a sensitivity beyond the standard quantum limit.

==> defs_thesis.tex <==
\newcommand {\tbf}[1] {\textbf{#1}}
\newcommand {\tit}[1] {\textit{#1}}
\newcommand {\tmd}[1] {\textmd{#1}}
\newcommand {\trm}[1] {\textrm{#1}}
\newcommand {\tsc}[1] {\textsc{#1}}
\newcommand {\tsf}[1] {\textsf{#1}}
\newcommand {\tsl}[1] {\textsl{#1}}
\newcommand {\ttt}[1] {\texttt{#1}}
\newcommand {\tup}[1] {\textup{#1}}

\newcommand {\figwidth} {100mm}
\newcommand {\Ref}[1] {Reference~\cite{#1}}
\newcommand {\Sec}[1] {Section~\ref{#1}}
\newcommand {\Eq}[1] {Eq.~\ref{#1}}
\newcommand {\App}[1] {Appendix~\ref{#1}}
\newcommand {\Chap}[1] {Chapter~\ref{#1}}
\newcommand {\Fig}[1] {Figure~\ref{#1}}
%\newcommand {\etal} {\emph{~et~al.}}
\newcommand {\bul} {$\bullet$ }   % bullet
\newcommand {\fig}[1] {Figure~\ref{#1}}   % references Figure x
\newcommand {\imp} {$\Rightarrow$}   % implication symbol (default)
\newcommand {\impt} {$\Rightarrow$}   % implication symbol (text mode)
\newcommand {\impm} {\Rightarrow}   % implication symbol (math mode)
\newcommand {\vect}[1] {\mathbf{#1}}
\newcommand {\hvect}[1] {\hat{\mathbf{#1}}}
\newcommand {\del} {\partial}
\newcommand {\eqn}[1] {Equation~(\ref{#1})}
\newcommand {\tab}[1] {Table~\ref{#1}} % references Table x
%\newcommand {\half} {\frac{1}{2}}
\newcommand {\ten}[1] {\times10^{#1}}
%\newcommand {\bra}[2] {\mbox{}_{#2}\langle #1 |}
%\newcommand {\ket}[2] {| #1 \rangle_{#2}}
\newcommand {\Bra}[2] {\mbox{}_{#2}\left.\left\langle #1 \right.\right|}
\newcommand {\Ket}[2] {\left.\left| #1 \right.\right\rangle_{#2}}
\newcommand {\im} {\mathrm{Im}}
\newcommand {\re} {\mathrm{Re}}
\newcommand {\braket}[4] {\mbox{}_{#3}\langle #1 | #2 \rangle_{#4}}
\newcommand {\dotprod}[4] {\mbox{}_{#3}\langle #1 | #2 \rangle_{#4}}
\newcommand {\trace}[1] {\text{tr}\left(#1\right)}

\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\bmat}{\begin{pmatrix}}
\newcommand{\emat}{\end{pmatrix}}

\newcommand{\natc}{N@C$_{60}$}
\newcommand{\natcseventy}{N@C$_{70}$}
\newcommand{\heatc}{He@C$_{60}$}
\newcommand{\heatcseventy}{He@C$_{70}$}
\newcommand{\patc}{P@C$_{60}$}

\newcommand{\csixty}{C$_{60}$}
\newcommand{\cseventy}{C$_{70}$}
\newcommand{\ceightyfour}{C$_{84}$}
\newcommand{\ceightytwo}{C$_{82}$}
\newcommand{\ceighty}{C$_{80}$}
\newcommand{\cseventyeight}{C$_{78}$}
\newcommand{\cseventysix}{C$_{76}$}
\newcommand{\mus}{$\rm{\mu}$s}
\newcommand{\cstwo}{CS$_2$}
\newcommand{\stwocltwo}{S$_2$Cl$_2$}

\newcommand{\nfourteen}{$^{14}$N}
\newcommand{\ptone}{$^{31}$P}
\newcommand{\nfifteen}{$^{15}$N}
\newcommand{\cthirteen}{$^{13}$C}
\newcommand{\oneh}{$^{1}$H}
\newcommand{\twoh}{$^{2}$D}

\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
%\newcommand{\e}{\mbox{e}}
\newcommand{\w}{\omega}
\newcommand{\thetai}{\theta_i}
\newcommand{\raiz}{\mbox{$\textstyle \frac{1}{\sqrt{2}}$}}
\newcommand{\ket}[1]{\left| #1 \right\rangle}
\newcommand{\bra}[1]{\left\langle #1 \right|}
\newcommand{\proj}[1]{\ket{#1}\bra{#1}}
\newcommand{\av}[1]{\langle #1\rangle}
\newcommand{\inprod}[2]{\braket{#1}{#2}}
\newcommand{\upket}{\ket{\uparrow}}
\newcommand{\downket}{\ket{\downarrow}}

%journal titles
\newcommand{\ACIE}{Ang. Chem. Int. Ed.}
\newcommand{\APL}{Appl. Phys. Lett.}
\newcommand{\CCOMM}{Chem. Comm.}
\newcommand{\CPL}{Chem. Phys. Lett.}
\newcommand{\IJTP}{Int. J. Thermophys.}
\newcommand{\JCP}{J. Chem. Phys.}
\newcommand{\JAP}{J. Appl.. Phys.}
\newcommand{\JACS}{J. Am. Chem. Soc.}
\newcommand{\JMOLLIQ}{J. Mol. Liq.}
\newcommand{\JMR}{J. Mag. Res.}
\newcommand{\JPC}{J. Phys. Chem.}
\newcommand{\JPCM}{J. Phys. Cond. Matt.}
\newcommand{\MOLPHYS}{Mol. Phys.}
\newcommand{\PCCP}{Phys. Chem. Chem. Phys.}
\newcommand{\PTRSA}{Phil.~Trans.~R.~Soc. A}
\newcommand{\PR}{Phys. Rev.}
\newcommand{\PRA}{Phys. Rev. A}
\newcommand{\PRB}{Phys. Rev. B}
\newcommand{\PRL}{Phys. Rev. Lett.}
\newcommand{\PNAS}{Proc. Natl. Acad. Sci.}
\newcommand{\RSI}{Rev. Sci. Inst.}

\newcommand{\tr}{$t_{\rm{r}}$}
\newcommand{\ttwo}{T$_2$}
\newcommand{\ttwoi}{T$_{2,i}$}
\newcommand{\ttwoo}{T$_{2,o}$}
\newcommand{\tonei}{T$_{1,i}$}
\newcommand{\toneo}{T$_{1,o}$}
\newcommand{\tone}{T$_1$}
\newcommand{\tonen}{$T_{\rm{1n}}$}
\newcommand{\tonee}{$T_{\rm{1e}}$}
\newcommand{\ttwon}{$T_{\rm{2n}}$}
\newcommand{\ttwoe}{$T_{\rm{2e}}$}
\newcommand{\tstore}{$T_{\rm{store}}$}
\newcommand{\ttwoq}{\rm{T}_2}
\newcommand{\toneq}{\rm{T}_1}
\newcommand{\ttwoiq}{\rm{T}_{2,\emph{i}}}
\newcommand{\ttwooq}{\rm{T}_{2,\emph{o}}}
\newcommand{\toneiq}{\rm{T}_{1,\emph{i}}}
\newcommand{\toneoq}{\rm{T}_{1,\emph{o}}}
\newcommand{\tw}{t_{\textrm{wait}}}

